jsCoq: Towards Hybrid Theorem Proving Interfaces

We describe jsCcoq, a new platform and user environment for the Coq interactive proof assistant. The jsCoq system targets the HTML5-ECMAScript 2015 specification, and it is typically run inside a standards-compliant browser, without the need of external servers or services. Targeting educational use, jsCoq allows the user to start interaction with proof scripts right away, thanks to its self-contained nature. Indeed, a full Coq environment is packed along the proof scripts, easing distribution and installation. Starting to use jsCoq is as easy as clicking on a link. The current release ships more than 10 popular Coq libraries, and supports popular books such as Software Foundations or Certified Programming with Dependent Types. The new target platform has opened up new interaction and display possibilities. It has also fostered the development of some new Coq-related technology. In particular, we have implemented a new serialization-based protocol for interaction with the proof assistant, as well as a new package format for library distribution.

==> eptcsdata.tex <==
\providecommand{\firstpage}{15}
\providecommand{\publicationstatus}{Autexier, S. and Quaresma, P. (Eds.): Proceedings of 12th\\ International Workshop on User Interfaces for Theorem Provers (UITP 2016)\\
EPTCS 239, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.239.2}{10.4204/EPTCS.239.2}}
\pdfoutput=1

